Divergence-Augmented Policy Optimization

In deep reinforcement learning, policy optimization methods need to deal with issues such as function approximation and the reuse of off-policy data. Standard policy gradient methods do not handle off-policy data well, leading to premature convergence and instability. This paper introduces a method to stabilize policy optimization when off-policy data are reused. The idea is to include a Bregman divergence between the behavior policy that generates the data and the current policy to ensure small and safe policy updates with off-policy data. The Bregman divergence is calculated between the state distributions of two policies, instead of only on the action probabilities, leading to a divergence augmentation formulation. Empirical experiments on Atari games show that in the data-scarce scenario where the reuse of off-policy data becomes necessary, our method can achieve better performance than other state-of-the-art deep reinforcement learning algorithms.

==> analysis.tex <==

For simplicity, we define 
\[
V(\theta) = \langle r, \mu_{\pi_\theta} \rangle = \E_{s,a\sim d_\pi \pi} r(s,a),
\] and conditional KL-divergence 
\[
D(\theta, \theta_t) = \E_{s\sim d_\theta} \log\frac{\pi_{\theta}(a|s)}{\pi_{\theta_t}(a|s)}
\]
Denote $A(s,a) = \mathcal{Q}^\pi(r)(s,a)$, $A'(s,a) = \mathcal{Q}^\pi(\nabla D_\text{KL}(\mu_\pi, \pi_t))$. The original policy loss can be written as
\[
g_1(s,a|\theta, \theta_t) = \E_{(s,a)\sim \pi_t d_{\pi_t}} \frac{d_\pi(s)}{d_{\pi_t}(s)} \frac{\pi(a|s)}{\pi_t(a|s)} (A(s,a) - \lambda A'(s,a)) \nabla_\theta\log\pi(a|s)
\]
In practice, we omit the state ratio of $d_\pi / d_{\pi_t}$, resulting in
\[
g_2(s,a|\theta, \theta_t) = \E_{(s,a)\sim \pi_t d_{\pi_t}} \frac{\pi(a|s)}{\pi_t(a|s)} (A(s,a) - \lambda A'(s,a)) \nabla_\theta\log\pi(a|s)
\]
In the first proposition, we show that the bias introduced by omitting the state ratio can be bounded by the conditional KL divergence. Specifically, we have
\begin{prop}
Under regularity conditions, the norm of bias of gradient can be bounded by the conditional KL-divergence:
\[
\lVert g_1(\cdot|\theta, \theta_t) - g_2(\cdot|\theta, \theta_t) \rVert^2 \le c D(\theta, \theta_t)
\]
\end{prop}
The proof can be found in Appendix, which follows from bounding the difference of $d_\pi$ and $d_{\pi_t}$.

which is sufficient for the local convergence of $V(\theta)$.
Consider the outer iteration from $\theta_{t-1}$ to $\theta_t$
\[
\theta_t = \argmin_{\theta} V(\theta) - \lambda D(\theta, \theta_{t-1})
\]
which is solved approximately by the inner iteration starting from $\psi_0 = \theta_{t_1}$ and
\begin{align}
    \psi_{i+1} = \psi_{i} + \frac{\eta}{m} g_2(\cdot|\psi_{i}, \theta_{t-1}), \quad i = 0, \cdots, m-1, \label{eq:incre-update-1}
\end{align}
and finally setting $\theta_t = \psi_m$.
In the next proposition, we \red{hopefully} claim that $V(\theta)$ converges locally
\begin{prop}
With iteration defined in (\ref{eq:incre-update-1}), we \red{hopefully} have
\[
V(\theta_t) \ge V(\theta_{t-1}) + C \lVert \nabla V(\theta_{t+1}) \rVert^2
\]
which is sufficient for the local convergence of $V(\theta)$.
\end{prop}


==> instructions.tex <==

\section{Submission of papers to NeurIPS 2019}

NeurIPS requires electronic submissions.  The electronic submission site is
\begin{center}
  \url{https://cmt.research.microsoft.com/NeurIPS2019/}
\end{center}

Please read the instructions below carefully and follow them faithfully.

\subsection{Style}

Papers to be submitted to NeurIPS 2019 must be prepared according to the
instructions presented here. Papers may only be up to eight pages long,
including figures. Additional pages \emph{containing only acknowledgments and/or
  cited references} are allowed. Papers that exceed eight pages of content
(ignoring references) will not be reviewed, or in any other way considered for
presentation at the conference.

The margins in 2019 are the same as since 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.

Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.

\subsection{Retrieval of style files}

The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2019.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.

The only supported style file for NeurIPS 2019 is \verb+neurips_2019.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}

The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.

\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.

At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.

The file \verb+neurips_2019.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.

The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2019+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2019}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %
   \newcommand{\Nat}{I\!\!N} %
   \newcommand{\CC}{I\!\!\!\!C} %
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\subsubsection*{Acknowledgments}

Use unnumbered third level headings for the acknowledgments. All acknowledgments
go at the end of the paper. Do not include acknowledgments in the anonymized
submission, only in the final paper.

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references. {\bf Remember that you can use more than eight
  pages as long as the additional pages contain \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.


==> misc.tex <==
\section{Alternative formulation} \label{secerrl}

Instead of using mirror descent formulation, We consider the divergence-augmented policy optimization problem as solving original reinforcement learning problem with divergence-augmented return, following various prior work (\cite{ziebart2010modeling,fox2015taming,haarnoja2017reinforcement,nachum2017bridging, schulman2017equivalence}).
Specifically, let us define the \textit{divergence-augmented return} to be $\sum_{t=0}^{\infty} \gamma^t \left(r_t - \temp \log \frac{\pi(a_t|s_t)}{\piref(a_t|s_t)}\right)$ and the new optimization objective as its expectation over the policy-induced trajectory to be 
\begin{align}
\tilde{J}(\pi)=
\E_{\tau|\pi} \left[\sum_{t=0}^{\infty} \gamma^t \left(r_t - \temp \log \frac{\pi(a_t|s_t)}{\piref(a_t|s_t)}\right)\right]
=
\E_{\tau|\pi} \left[\sum_{t=0}^{\infty} \gamma^t \left(r_t - \temp\KL_t \right)\right]
\end{align}
where $r_t$ is the reward, $\gamma \in [0,1]$ is the discount factor,
$\temp$ is a scalar temperature coefficient, 
and $\KL_t$ is the Kullback-Leibler divergence between the current policy $\pi$ and a reference policy $\piref$ at timestep $t$: $\KL_t = \kl{\pi(\cdot \given s_t)}{\piref(\cdot \given s_t)}$.
We will sometimes use the notation $\KL(s) = \kl{\pi}{\piref}(s) = \kl{\pi(\cdot \given s)}{\piref(\cdot \given s)}$.
To emulate the effect of a standard entropy bonus (up to a constant), one can define $\piref$ to be the uniform distribution.
The subsequent sections will generalize some of the concepts from reinforcement learning to the setting where we are maximizing the entropy-augmented discounted return.

\subsection{Value Functions}
We are obliged to alter our definitions of value functions to include the new KL penalty terms.
We shall define the state-value function as the expected return:
\begin{align}
\Vpi(s) = 
\Ea{\sum_{t=0}^{\infty} \gamma^t \left(r_t - \temp \log \frac{\pi(a_t|s_t)}{\piref(a_t|s_t)}\right) \givenb s_0=s}
=\Ea{\sum_{t=0}^{\infty} \gamma^t \left(r_t - \temp \KL_t\right) \givenb s_0=s} \label{vpidef}
\end{align}
and we shall define the $Q$-function as
\begin{align}
\Qpi(s, a) &= 
\Ea{r_0 + \sum_{t=1}^{\infty} \gamma^t \left(r_t - \temp \log \frac{\pi(a_t|s_t)}{\piref(a_t|s_t)} \right) \givenb s_0=s, a_0=a} \\
&=
\Ea{r_0 + \sum_{t=1}^{\infty} \gamma^t \left(r_t - \temp \KL_t \right) \givenb s_0=s, a_0=a} \label{qpidef}
\end{align}
Note that this $Q$-function does not include the first KL penalty term, which does not depend on the action $a_0$.
This definition makes some later expressions simpler, and it leads to the following relationship between $\Qpi$ and $\Vpi$:
\begin{align}
\Vpi(s)
&= \Eb{a \sim \pi}{\Qpi(s,a)} - \temp \KL(s),
\end{align}
which follows from matching terms in the sums in \Cref{vpidef,qpidef}.
\subsection{Boltzmann Policy}
With entropy regularization, we need to alter our notion of a greedy policy, as the optimal policy is stochastic.
Since $\Qpi$ omits the first entropy term, it is natural to define the following stochastic policy, which is called the Boltzmann policy, and is analogous to the greedy policy:
\begin{align}
\pibolq(\cdot \given s)
&= \argmax_{\pi} \lrbrace*{ \Eb{a \sim \pi}{Q(s,a)} - \tau \kl{\pi}{\piref}(s)}\\
&= \piref(a \given s) \exp(Q(s,a)/\tau) / \underbrace{\Eb{a' \sim \piref}{\exp(Q(s,a')/\tau)}}_{\text{normalizing constant}}.
\end{align}
where the second equation is analogous to \Cref{pistardef} from the bandit setting.

Also analogously to the bandit setting, it is natural to define $V_Q$ (a function of $Q$) as
\begin{align}
V_Q(s) = \tau \log \Eb{a' \sim \piref}{\exp(Q(s,a')/\tau)}
\end{align}
so that
\begin{align}
\pibolq(a \given s) = \piref(a \given s) \exp((Q(s,a) - V_Q(s))/\tau) \label{boltz-def}
\end{align}
Under this definition, it also holds that
\begin{align}
V_Q(s) = \Eb{a \sim \pibolq(s)}{Q(s,a)} - \tau \kl{\pibolq}{\piref}(s) \label{mdpvid}
\end{align}
in analogy with \Cref{banditvthid}.
Hence, $V_Q(s)$ can be interpreted as an estimate of the expected entropy-augmented return, under the Boltzmann policy $\pibolq$.

Another way to interpret the Boltzmann policy is as the exponentiated advantage function.
Defining the advantage function as $A_Q(s,a) = Q(s,a) - V_Q(s)$, \Cref{boltz-def} implies that $\frac{\pibolq(a \given s)}{\piref(a \given s)} = \exp(A_Q(s,a)/\tau)$.

\subsection{Fixed-Policy Backup Operators}

The $\Tpi$ operators (for $Q$ and $V$) in standard reinforcement learning correspond to computing the expected return with a one-step lookahead: they take the expectation over one step of dynamics, and then fall back on the value function at the next timestep.
We can easily generalize these operators to the entropy-regularized setting.
We define
\begin{align}
[\Tpi V](s) &= \Eb{a\sim \pi,(r, s') \sim P(r, s' \given s, a)}{r - \tau \KL(s) + \gamma V(s')} \label{vtpi}\\
[\Tpi Q](s, a) &= \Eb{(r, s') \sim P(r, s' \given s, a)}{r + \gamma (\Eb{a' \sim \pi}{Q(s',a')} - \tau \KL(s'))}. \label{qtpi}
\end{align}

Repeatedly applying the $\Tpi$ operator $(\Tpi^n V = \underbrace{\Tpi(\Tpi(\dots \Tpi}_{\text{$n$ times}}(V))))$ corresponds to computing the expected return with a multi-step lookahead. That is, repeatedly expanding the definition of $\Tpi$, we obtain
\begin{align}
&[\Tpi^n V](s)=\Ea{\sum_{t=0}^{n-1}\gamma^t (r_t - \tau \KL_t)  + \gamma^n V(s_n) \givenb s_0=s}\\
&[\Tpi^n Q](s,a) - \tau \K(s) = \Ea{\sum_{t=0}^{n-1} \gamma^t (r_t - \tau \KL_t)  + \gamma^n (Q(s_n, a_n) - \tau \KL_n) \givenb s_0=s, a_0=a}. \label{qtpin}
\end{align}
As a sanity check, note that in both equations, the left-hand side and right-hand side correspond to estimates of the total discounted return $\sum_{t=0}^{\infty} \gamma^t (r_t - \tau \KL_t)$.

The right-hand side of these backup formulas can be rewritten using ``Bellman error'' terms $\delta_t$.
To rewrite the state-value ($V$) backup, define
\begin{align}
\delta_t = (r_t - \tau\KL_t) + \gamma V(s_{t+1}) - V(s_t) \label{deltadef}
\end{align}
Then we have
\begin{align}
[\Tpi^n V](s)=\Ea{\sum_{t=0}^{n-1}\gamma^t \delta_t  + \gamma^n V(s_n) \givenb s_0=s}.
\end{align}

\subsection{Boltzmann Backups}
We can define another set of backup operators corresponding to the Boltzmann policy, $\pi(a \given s) \propto \piref(a \given s) \exp(Q(s,a)/\tau)$.
We define the following Boltzmann backup operator:
\begin{align}
[\T Q](s,a) &= \Eb{(r,s') \sim P(r,s' \given s,a)}{r + \gamma \underbrace{\Eb{a' \sim \G Q}{Q(s,a)} - \tau \kl{\G Q}{\piref}(s')}_{(\ast)}}\\
&=\Eb{(r,s') \sim P(r,s' \given s,a)}{r + \gamma \underbrace{\tau \log \Eb{a'\sim\piref}{\exp(Q(s',a')/\tau)}}_{(\ast\ast)}}
\end{align}
where the simplification from $(\ast)$ to $(\ast\ast)$ follows from the same calculation that we performed in the bandit setting (\Cref{banditvdef,banditvthid}).


The $n$-step operator $\Tpi^n$ for $Q$-functions also simplifies in the case that we are executing the Boltzmann policy.
Starting with the equation for $\Tpi^n Q$ (\Cref{qtpin}) and setting $\pi=\pibolq$, and then using \Cref{mdpvid} to rewrite the expected $Q$-function terms in terms of $V_Q$, we obtain
\begin{align}
[(\T_{\pibolq})^n Q](s,a) - \tau \K(s)
&= \Ea{\sum_{t=0}^{n-1} \gamma^t (r_t - \tau \KL_t)  + \gamma^n (Q(s_n, a_n) - \tau \KL_n) \givenb s_0=s, a_0=a}\\
&= \Ea{\sum_{t=0}^{n-1} \gamma^t (r_t - \tau \KL_t)  + \gamma^n V_Q(s_n) \givenb s_0=s, a_0=a}.
\end{align}
From now on, let's denote this $n$-step backup operator by $\T_{\pibol, n}$. (Note $T_{\pibolq,n} \neq \T^n Q$, even though $\T_{\pibolq,1}Q=\T Q$, because $\T_{\pibolq}$ depends on $Q$.)


One can similarly define the \tdlam{} version of this backup operator
\newcommand{\Tpibol}{\T_{\pibolq}}
\newcommand{\Tpibollam}{\T_{\pibolq, \lambda}}
\newcommand{\Tpiboln}{\T_{\pibolq, n}}
\begin{align}
[\Tpibollam Q] = (1-\lambda)(1 + \lambda \Tpibol + (\lambda \Tpibol)^2 + \dots) \Tpibol Q. \label{tbollam}
\end{align}
One can straightforwardly verify by comparing terms that it satisfies
\begin{align}
&[\Tpibollam Q](s,a) = Q(s,a) + \Ea{\sum_{t=0}^{\infty} (\gamma \lambda)^t \delta_t \givenb s_0=s, a_0=a},\nonumber\\
&\where \delta_t = (r_t - \temp \KL_t) + \gamma V_Q(s_{t+1}) - V_Q(s_t).
\label{eq:qlambackup}
\end{align}



\subsection{Soft \titleQ-Learning} \label{softq}
The Boltzmann backup operators defined in the preceding section can be used to define practical variants of $Q$-learning that can be used with nonlinear function approximation.
These methods, which optimize the entropy-augmented return, will be called soft $Q$-learning.
Following \cite{mnih2015human}, modern implementations of $Q$-learning, and $n$-step $Q$-learning (see \cite{mnih2016asynchronous}) update the $Q$-function incrementally to compute the backup against a fixed target $Q$-function, which we'll call $\Qtarg$.
In the interval between each target network update, the algorithm is approximately performing the backup operation $Q \leftarrow \T \Qtarg$ ($1$-step) or $Q \leftarrow \T_{\pibol_{\Qtarg},n} \Qtarg$ ($n$-step). To perform this approximate minimization, the algorithms minimize the least squares loss
\begin{alignat}{2}
L(Q) &= \Eb{t, s_t,a_t}{\half (Q(s_t, a_t) - y_t)^2}, \where \\
y_t &= r_t + \gamma V_{\Qtarg}(s_{t+1}) \qquad &&\text{1-step $Q$-learning} \label{1step}\\
y_t &= \tau \KL_t + \sum_{d=0}^{n-1} \gamma^d (r_{t+d} - \tau \KL_{t+d}) + \gamma^{n} V_{\Qtarg}(s_{t+n}) \qquad &&\text{$n$-step $Q$-learning}    \label{nstep} \\
&= \tau \KL_t + V_{\Qtarg}(s_t) + \sum_{d=0}^{n-1} \gamma^d \delta_{t+d} \nonumber \\
&\where \delta_t = (r_t - \tau \KL_t) + \gamma V_{\Qtarg}(s_{t+1}) - V_{\Qtarg}(s_t) \label{nstepq-target}
\end{alignat}
In one-step $Q$-learning (\Cref{1step}), $y_t$ is an unbiased estimator of $[\T Q](s_t, a_t)$, regardless of what behavior policy was used to collect the data.
In $n$-step $Q$-learning (\Cref{nstep}), for $n>1$, $y_t$ is only an unbiased estimator of $[\T_{\pibol_{\Qtarg},n} \Qtarg](s_t, a_t)$ if actions $a_t, a_{t+1}, \dots, a_{t+d-1}$ are sampled using $\pibol_{\Qtarg}$.
\subsection{Policy Gradients} \label{entpg}

Entropy regularization is often used in policy gradient algorithms, with gradient estimators of the form
\begin{align}
\Eb{t, s_t, a_t}{\gradth \log \pith(a_t \given s_t) \sum_{t' \ge t} r_{t'} - \temp \gradth \kl{\pith}{\piref}(s_t)} \label{naivepg}
\end{align}
(\cite{williams1992simple,mnih2016asynchronous}).

However, these are not proper estimators of the entropy-augmented return $\sum_{t} (r_t - \temp \KL_t)$, since they don't account for how actions affect entropy at future timesteps.
Intuitively, one can think of the KL terms as a cost for ``mental effort''. \Cref{naivepg} only accounts for the instantaneous effect of actions on mental effort, not delayed effects.

To compute proper gradient estimators, we need to include the entropy terms in the return.
We will define the discounted policy gradient in the following two equivalent ways---first, in terms of the empirical return; second, in terms of the value functions $\Vpi$ and $\Qpi$:
\begin{align}
g_{\gamma}(\pith)
&= \Ea{\sum_{t=0}^{\infty} \gradth \log \pith(a_t \given s_t) \lrparen*{r_0 + \sum_{d=1}^{\infty} \gamma^{d} (r_{t+d}-\temp\KL_{t+d}) - \temp \gradth \kl{\pith}{\piref}(s_t)}} \\
&= \Ea{\sum_{t=0}^{\infty} \gradth \log \pith(a_t \given s_t) (\Qpi(s_t, a_t)- \Vpi(s_t) ) - \temp \gradth \kl{\pith}{\piref}(s_t)}
\end{align}
\begin{minipage}{.5\textwidth}
In the special case of a finite-horizon problem---i.e., $r_t=\KL_t=0$ for all $t \ge T$---the undiscounted ($\gamma=1$) return is finite, and it is meaningful to compute its gradient.
In this case, $g_1(\pith)$ equals the undiscounted policy gradient:
\begin{align}
g_{1}(\pi) = \gradth \Ea{\sum_{t=0}^{T-1}(r_t - \temp \KL_t)}
\end{align}
This result is obtained directly by considering the stochastic computation graph for the loss (\cite{schulman2015gradient}), shown in the figure on the right. The edges from $\theta$ to the KL loss terms lead to the $\gradth \kl{\pith}{\piref}(s_t)$ terms in the gradient; the edges to the stochastic actions $a_t$ lead to the $\gradth \log \pith(a_t \given s_t) \sum_{t=d}^{T-1} (r_{t+d} - \tau \KL_{t+d})$ terms in the gradient.
\end{minipage}
\begin{minipage}{.5\textwidth}
\begin{center}
\includegraphics[height=.8\textwidth]{figures/pg-entreg.pdf}
\end{center}
\end{minipage}

Since $g_1(\pith)$ computes the gradient of the entropy-regularized return, one interpretation of $\ggam(\pith)$ is that it is an approximation of the undiscounted policy gradient $g_1(\pith)$, but that it allows for lower-variance gradient estimators by ignoring some long-term dependencies.
A different interpretation of $\ggam(\pi)$ is that it gives a gradient flow such that $\pistar=\pibol_{\Qstar}$ is the (possibly unique) fixed point.

As in the standard MDP setting, one can define approximations to $\ggam$ that use a value function to truncate the returns for variance reduction.
These approximations can take the form of $n$-step methods (\cite{mnih2016asynchronous}) or \tdlam{}-like methods (\cite{schulman2015high}), though we will focus on $n$-step returns here.
Based on the definition of $\ggam$ above, the natural choice of variance-reduced estimator is
\begin{align}
\Eb{t, s_t, a_t}{\gradth \log \pith(a_t \given s_t) \sum_{d=0}^{n-1} \gamma^d \delta_{t+d} } \label{nsteppg}
\end{align}
where $\delta_t$ was defined in \Cref{deltadef}.


The state-value function $V$ we use in the above formulas should approximate the entropy augmented return $\sum_{t=0}^{\infty}\gamma^t (r_t - \tau \KL_t)$.
We can fit $V$ iteratively by approximating the $n$-step backup $V \leftarrow \Tpi^n V$, by minimizing a squared-error loss
\begin{align}
&L(V) = \Eb{t, s_t}{\half (V(s_t) - y_t)^2},\\
&\where y_t = \sum_{d=0}^{n-1} \gamma^d r_{t+d} + \gamma^d V(s_{t+d}) = V(s_t) + \sum_{d=0}^{n-1} \gamma^d \delta_{t+d}. \label{vtarg}
\end{align}


==> theoretical.tex <==

\begin{align} \label{eq:consistency}
\nabla F(x) - \eta \nabla \ell(x) \in \red{\D^*\text{(definition)}} \qquad \forall (x,\ell) \in \left(\K \cap \D\right) \times 
\red{\L~\text{(subdifferentiable functions)}}~. 
\end{align}





\begin{thm}[Regret of OMD with a Legendre function \citep{bubeck2012regret}] \label{th:MGD}
Let $\K$ \red{($\Delta_\Pi$)} be a compact and convex set of arms, $\L$  be a set of subdifferentiable \red{(linear $\ell_t(\mu) = -\langle r, \mu \rangle$)} functions, and $F$ a Legendre function defined on $\D \supset \K$ \red{($\Delta(\mathcal{S}\times\mathcal{A}) \supset \Delta_\Pi$)}, such that \eqref{eq:consistency} is satisfied. Then OMD satisfies for any $x \in \K$ \red{($\mu \in \Delta_\Pi$)},
\begin{align*}
\sum_{t=1}^n \ell_t(x_t) - \sum_{t=1}^n \ell_t(x)
& \leq \frac{F(x) - F(x_1)}{\eta} \\
&  \quad + \frac{1}{\eta} \sum_{t=1}^n D_{F^*}\bigg(\nabla F(x_t) - \eta \nabla \ell_t(x_t), \nabla F(x_t)\bigg)~.
\end{align*}
\red{
\begin{align*}
\sum_{t=1}^n \ell_t(\mu_t) - \sum_{t=1}^n \ell_t(\mu)
& \leq \frac{F(\mu) - F(\mu_1)}{\eta} \\
&  \quad + \frac{1}{\eta} \sum_{t=1}^n D_{F^*}\bigg(\nabla F(\mu_t) - \eta \nabla \ell_t(\mu_t), \nabla F(\mu_t)\bigg)~.
\end{align*}
}

\end{thm}
\begin{proof}
Let $x \in \K$. Since $\L$ is a set of subdifferentiable \red{(linear)} functions, we have:
$$\sum_{t=1}^n \left( \ell_t(x_t) - \ell_t(x) \right) \leq \sum_{t=1}^n \nabla \ell_t(x_t)^{\top} (x_t -x)~.$$
\red{$$\sum_{t=1}^n \left( \ell_t(\mu_t) - \ell_t(\mu) \right) = \sum_{t=1}^n \nabla \ell_t(\mu_t)^{\top} (\mu_t - \mu)~.$$
}
Using \eqref{eq:mirrormap}, and applying the definition of $D_F$, one obtains
  \begin{align*}
  \eta \nabla \ell_t(x_t)^{\top} (x_t - x) & = (x-x_t)^{\top} \big(\nabla F(w_{t+1}) - \nabla F(x_t) \big)\\
  & = D_F(x,x_t)+D_F(x_t,w_{t+1})-D_F(x,w_{t+1})~.
  \end{align*}
\red{
  \begin{align*}
  \eta \nabla \ell_t(\mu_t)^{\top} (\mu_t - \mu) & = (\mu - \mu_t)^{\top} \big(\nabla F(\tilde{\mu}_{t+1}) - \nabla F(\mu_t) \big)\\
  & = D_F(\mu,\mu_t)+D_F(\mu_t, \tilde{\mu}_{t+1})-D_F(\mu, \tilde{\mu}_{t+1})~.
  \end{align*}
}
By \red{Generalized Pythagorean Theorem}, one gets 
  $D_F(x,w_{t+1}) \ge D_F(x,x_{t+1}) + D_F(x_{t+1},w_{t+1}),$ 
  \red{$D_F(\mu,\tilde{\mu}_{t+1}) \ge D_F(\mu,\mu_{t+1}) + D_F(\mu_{t+1},\tilde{\mu}_{t+1}),$~}hence
  \begin{align*}
  \eta \nabla \ell_t(x_t)^{\top} (x_t - x) & \le D_F(x,x_t)+D_F(x_t,w_{t+1}) \\
& \quad -D_F(x,x_{t+1})-D_F(x_{t+1},w_{t+1})~.
  \end{align*}
\red{
  \begin{align*}
  \eta \nabla \ell_t(\mu_t)^{\top} (\mu_t - \mu) & \le D_F(\mu,\mu_t)+D_F(\mu_t, \tilde{\mu}_{t+1}) \\
& \quad -D_F(\mu, \mu_{t+1})-D_F(\mu_{t+1}, \tilde{\mu}_{t+1})~.
  \end{align*}
}
Summing over $t$ then gives  
  \begin{align*}
  \sum_{t=1}^n \eta \nabla \ell_t(x_t)^{\top} (x_t - x) & \le D_F(x,x_1)-D_F(x,x_{n+1}) \\
& \quad +\sum_{t=1}^n \big(D_F(x_t,w_{t+1}) -D_F(x_{t+1},w_{t+1})\big)~.
  \end{align*}
\red{
  \begin{align*}
  \sum_{t=1}^n \eta \nabla \ell_t(\mu_t)^{\top} (\mu_t - \mu) & \le D_F(\mu, \mu_1)-D_F(\mu, \mu_{n+1}) \\
& \quad +\sum_{t=1}^n \big(D_F(\mu_t, \tilde{\mu}_{t+1}) -D_F(\mu_{t+1}, \tilde{\mu}_{t+1})\big)~.
  \end{align*}
}
By the nonnegativity of the Bregman divergences, we get 
$$\sum_{t=1}^n \eta \nabla \ell_t(x_t)^{\top} (x_t - x)
\le D_F(x,x_1)+\sum_{t=1}^n D_F(x_t,w_{t+1})~.$$
\red{
$$\sum_{t=1}^n \eta \nabla \ell_t(\mu_t)^{\top} (\mu_t - \mu)
\le D_F(\mu, \mu_1)+\sum_{t=1}^n D_F(\mu_t, \tilde{\mu}_{t+1})~.$$
}
If $F$ is a Legendre function, one has
  $
  D_F(x_t,w_{t+1})=D_{F^*}\big(\nabla F(x_t)- \eta \nabla \ell_t(x_t),\nabla F(x_t)\big)
  $
\red{
  $
  D_F(\mu_t, \tilde{\mu}_{t+1}) = D_{F^*}\big(\nabla F(x_t)- \eta \nabla \ell_t(x_t),\nabla F(x_t)\big)
  $
}
and, moreover, by first-order optimality, one has $D_F(x,x_1) \leq F(x) - F(x_1)$, which concludes the proof.
\end{proof}
\red{
Note that here the pseudo-regret for OSMD is defined as
\begin{align}
    \bar{R}_n = \E \sum_{t=1}^n \tilde{\ell}_{t, I_t} - \min_{\mu \in \Delta_\Pi} \E \sum_{t=1}^n \ell_t(\mu)\\
    \bar{R}_n = \sum_{t=1}^n  \max_\pi J(\pi) - \sum_{t=1}^n J(\pi_t),
\end{align}
}
\begin{thm}[Pseudo-regret of OSMD \citep{bubeck2012regret}] \label{th:OSMD2}
Let $\K$ \red{($\Delta_\Pi$)} be a compact and convex set, $\L$ a set of subdifferentiable \red{(linear)} functions, and $F$ a Legendre function defined on $\D \supset \K$~ \red{($\Delta(\mathcal{S}\times\mathcal{A}) \supset \Delta_\Pi$)}. If OSMD is run with a loss estimate $\tilde{g}_t$ such that~\eqref{eq:consistency} is satisfied (with $\nabla \ell_t(x)$ \red{($\nabla \ell_t(\mu)$)} replaced by $\tilde{g}_t$, and with $\E\left[\tilde{g}_t \mid x_t\right] =\nabla \ell_t(x_t)$~\red{($\E\left[\tilde{g}_t \mid \mu_t\right] =\nabla \ell_t(\mu_t)$)}, 
Moreover if the loss is linear, that is $\ell(x) = \ell^{\top} x$ with \red{$\E \left[\tilde{\ell}_{t, I_t} \mid \mu_t \right] = \ell_t(\mu_t)$)}, then
\begin{align*}
\bar{R}_n & \leq \frac{\sup_{x \in \K} F(x) - F(x_1)}{\eta} + \frac{1}{\eta} \sum_{t=1}^n \E\, D_{F^*}\left(\nabla F(x_t) - \eta \tilde{g}_t, \nabla F(x_t)\right) 
\end{align*}
\red{
\begin{align*}
\bar{R}_n & \leq \frac{\sup_{\mu \in \Delta_\Pi} F(\mu) - F(\mu_1)}{\eta} + \frac{1}{\eta} \sum_{t=1}^n \E\, D_{F^*}\left(\nabla F(\mu_t) - \eta \tilde{g}_t, \nabla F(\mu_t)\right) 
\end{align*}
}
\end{thm}
\begin{proof}
Using Theorem \ref{th:MGD} one directly obtains:
$$\E \sum_{t=1}^n \tilde{g}_t^{\top} (x_t - x) \leq \frac{F(x) - F(x_1)}{\eta} + \frac{1}{\eta} \sum_{t=1}^n \E\, D_{F^*} \left(\nabla F(x_t) - \eta \tilde{g}_t, \nabla F(x_t)\right)~.$$
\red{
$$\E \sum_{t=1}^n \tilde{g}_t^{\top} (\mu_t - \mu) \leq \frac{F(\mu) - F(\mu_1)}{\eta} + \frac{1}{\eta} \sum_{t=1}^n \E\, D_{F^*} \left(\nabla F(\mu_t) - \eta \tilde{g}_t, \nabla F(\mu_t)\right)~.$$
}
Moreover since $\E\left[\tilde{g}_t \mid x_t\right] =\nabla \ell_t(x_t)$
\red{~(
$\E\left[\tilde{g}_t \mid \mu_t\right] =\nabla \ell_t(\mu_t)$
 and $\E\left[\tilde{l}_{t,I_t} \mid \mu_t\right] = \ell_t(\mu_t)$)}, one has:
\begin{align*}
\E \sum_{t=1}^n \left( \ell_t(\tilde{x}_t) - \ell_t(x) \right) & = \E \sum_{t=1}^n \left( \ell_t(\tilde{x}_t) - \ell_t(x_t) + \ell_t(x_t) - \ell_t(x) \right) \\
& \leq \E \sum_{t=1}^n \norm{x_t - \tilde{x}_t} \norm{\tilde{g}_t}_* + \E \sum_{t=1}^n \nabla \ell_t(x_t)^{\top} (x_t - x) \\
& = \E \sum_{t=1}^n \norm{x_t - \tilde{x}_t} \norm{\tilde{g}_t}_* + \E \sum_{t=1}^n \tilde{g}_t^{\top} (x_t - x)
\end{align*}
\red{
\begin{align*}
\E \sum_{t=1}^n \left( \tilde{\ell}_{t,I_t} - \ell_t(\mu) \right) & = \E \sum_{t=1}^n \left( \tilde{\ell}_{t,I_t} - \ell_t(\mu_t) + \ell_t(\mu_t) - \ell_t(\mu) \right) \\
& = \E \sum_{t=1}^n \nabla \ell_t(x_t)^{\top} (x_t - x) \\
& = \E \sum_{t=1}^n \tilde{g}_t^{\top} (x_t - x)
\end{align*}
}
which concludes the proof of the first regret bound. The case of a linear loss follows very easily from the same computations.
\end{proof}

\begin{thm}[OSMD with negative entropy]
\label{th:osmdnegent}
If OSMD is run on $\K=\Delta_\Pi$ and $\bar{\D}=\Delta(\mathcal{S}\times\mathcal{A})$ with $d=|\mathcal{S}\times \mathcal{A}|$ and $F(\mu) = \sum_{i=1}^d \mu_i \ln \mu_i - \sum_{i=1}^d \mu_i$, select arm $I_t$ according to $\mu_t$ such that the expectation of the observed loss $\E\left[\tilde{l}_{t,I_t} \mid \mu_t \right] = \ell_t(\mu_t)$, and gradient estimates $\tilde{g}_t$, then
$$\bar{R}_n \leq \frac{1}{\eta}\ln d + \frac{\eta}{2} \sum_{t=1}^n \sum_{i=1}^d \E\left[\mu_t(i)\,\tilde{g}_t(i)^2\right]~.$$
In particular, with the unbiased estimate \eqref{eq:banditestimate} and $\eta= \sqrt{\frac{2}{nd}\ln d}$,
$$\bar{R}_n \leq  \sqrt{2 d n \ln d}~.$$
\end{thm}
\begin{proof}
First note that, by the concavity of $\ln x$:
$$F(\mu) - F(\mu_1) \leq \sum_{i=1}^d \mu_{1,i} \ln \frac{1}{\mu_{1,i}} \leq \ln \left( \sum_{i=1}^d \mu_{1,i} \frac{1}{\mu_{1,i}}\right) = \ln d~.$$
Moreover, straightforward computations give
$$D_{F^*}\bigg(\nabla F(\mu_t) - \eta \tilde{g}_t, \nabla F(\mu_t)\bigg) =\sum_{i=1}^d \mu_{t,i}\, \Theta\left(- \eta \tilde{g}_{t,i}\right)$$
where $\Theta : x \in \mathbb{R} \mapsto \exp(x) - 1 - x$. Using that $\Theta(x) \leq \frac{x^2}{2}$ for all $x \leq 0$, concludes the proof of the first inequality (since $\tilde{g}_{t,i} \geq 0$). The second inequality follows from
\[
    \mu_{t,i}\,\E\left[\tilde{g}_{t,i}^2 \mid \mu_t\right] = 
    \mu_{t,i} \frac{\E\left[\tilde{\ell}_{t,i}^2\right]}{\mu_{t,i}^2}\E\left[\mathbbm{1}\{I_t=i\} \mid \mu_t\right] \le 1
\]
where we assumed \red{deterministic feedback or zero variance such that $\E\left[\tilde{\ell}_{t,i}^2\right] = \ell_{t,i}^2 $} and used $\tilde{\ell}_{t,i} = \ell_{t,i} \in [0,1]$~.
\end{proof}

